The European Spallation Source neutrino Super Beam

In this Snowmass 2021 white paper, we summarise the Conceptual Design of the European Spallation Source neutrino Super Beam (ESSvSB) experiment and its synergies with the possible future muon based facilities, e.g. a Low Energy nuSTORM and the Muon Collider. The ESSvSB will benefit from the high power, 5 MW, of the European Spallation Source (ESS) LINAC in Lund-Sweden to produce the world most intense neutrino beam, enabling measurements to be made at the second oscillation maximum. Assuming a ten-year exposure, physics simulations show that the CP-invariance violation can be established with a significance of 5 sigma over more than 70% of all values of delta CP and with an error in the measurement of the delta CP angle of less than 8 degree for all values of delta CP. However, several technological and physics challenges must be further studied before achieving a final Technical Design. Measuring at the 2nd oscillation maximum necessitates a very intense neutrino beam with the appropriate energy. For this, the ESS proton beam LINAC, which is designed to produce the world's most intense neutron beam, will need to be upgraded to 10 MW power, 2.5 GeV energy and 28 Hz beam pulse repetition rate. An accumulator ring will be required for the compression of the ESS LINAC beam pulse from 2.86 ms to 1.3 mus. A high power target station facility will be needed to produce a well-focused intense (super) mu-neutrino beam. The physics performance of that neutrino Super Beam in conjunction with a megaton underground Water Cherenkov neutrino far detector installed at a distance of either 360 km or 540 km from the ESS, the baseline, has been evaluated.

==> conclusion.tex <==
\section{Conclusion}

Neutrino long baseline experiments have for many years tried to reduce the systematic errors. In order to be less dependent on systematic uncertainties and taking into account the relatively large value of the last measured mixing angle $\theta_{13}$, it is more advantageous to operate the future long baseline neutrino experiments for CP violation discovery and $\delta_{CP}$ parameter measurement, at baselines corresponding to the second, rather than the first, oscillation maximum.

\noindent For this, a high intensity proton driver is needed.
The ESS$\nu$SB project proposes to use the \SI{5}{\mega\watt} ESS proton linac to produce a very intense neutrino beam, and place the far detector in a distance corresponding to the second oscillation maximum. By using a $\sim$~\SI{500}{\kilo\ton} fiducial mass Cherenkov detector, ESS$\nu$SB can reach, for 10-year running, 70\%  $\delta_{CP}$ coverage with a 5~$\sigma$ significance. After discovering CP violation in the leptonic sector, ESS$\nu$SB can measure $\delta_{CP}$ with a precision lower than 8$^\circ$.\\

\noindent Moreover, this project has a high potential for future upgrades by using the muons produced at the same time than the neutrinos or by using another target station to collect both signs $\mu^+$ and  $\mu^-$ to be used by a future low energy nu STORM, Neutrino Factory or/and a Muon Collider.

\noindent In this document are reported the necessary modification of the ESS linac, the study of an accumulation ring to shorten the proton pulses from milliseconds level to microseconds. Extensive studies were also necessary concerning a target station able to afford the \SI{5}{\mega\watt} proton power and produce a competitive neutrino beam. To evaluate the physics performance of the project a design of a near and far detector are proposed. The position of the far detector has been chosen taking into account the physics performance but also the rock quality at this precise position situated near an active mine.\\

\noindent The overall cost of the project is estimated to be around 1.7~B€, with about 1~B€ devoted to the detectors.


